Results of the 2023 Census of Beat Saber Users: Virtual Reality Gaming Population Insights and Factors Affecting Virtual Reality E-Sports Performance

The emergence of affordable standalone virtual reality (VR) devices has allowed VR technology to reach mass-market adoption in recent years, driven primarily by the popularity of VR gaming applications such as Beat Saber. However, despite being the top-grossing VR application to date and the most popular VR e-sport, the population of over 6 million Beat Saber users has not yet been widely studied. In this report, we present a large-scale comprehensive survey of Beat Saber players (N=1,006) that sheds light on several important aspects of this population, including their background, biometrics, demographics, health information, behavioral patterns, and technical device specifications. We further provide insights into the emerging field of VR e-sports by analyzing correlations between responses and an authoritative measure of in-game performance.

==> 01-intro.tex <==
\section{Introduction}
% 01 - Introduction

% metaverse
% vr esports
